Long-range and hierarchical language predictions in brains and algorithms

Deep learning has recently made remarkable progress in natural language processing. Yet, the resulting algorithms remain far from competing with the language abilities of the human brain. Predictive coding theory offers a potential explanation to this discrepancy: while deep language algorithms are optimized to predict adjacent words, the human brain would be tuned to make long-range and hierarchical predictions. To test this hypothesis, we analyze the fMRI brain signals of 304 subjects each listening to 70min of short stories. After confirming that the activations of deep language algorithms linearly map onto those of the brain, we show that enhancing these models with long-range forecast representations improves their brain-mapping. The results further reveal a hierarchy of predictions in the brain, whereby the fronto-parietal cortices forecast more abstract and more distant representations than the temporal cortices. Overall, this study strengthens predictive coding theory and suggests a critical role of long-range and hierarchical predictions in natural language processing.

==> 21_intro_old.tex <==
% Recent progress in SSL 
\dropcap{I}n less than three years, deep language algorithms have made considerable progress in text generation, translation and completion \cite{vaswani_attention_2017,radford_language_nodate, brown_language_2020}, thanks to a simple learning rule: predicting words from adjacent context. 
%
% Predict brain activity 
Remarkably, the activations of these algorithms linearly map onto the human brain responses to spoken and written language (fMRI \cite{toneva_interpreting_2019, schrimpf_artificial_2020}, MEG \cite{toneva_interpreting_2019, caucheteux_language_2020} and ECoG \cite{goldstein_thinking_2021}), and this mapping closely relates to the algorithms' ability to predict incoming words \citep{caucheteux_language_2020,schrimpf_artificial_2020}.

% Limitations
Yet, the gap between machines and humans remains considerable: current language models remain poor at story generation, summarization, dialogue and long-form question answering \cite{holtzman_curious_2020, wiseman_challenges_2017, thakur_beir_2021, raffel_exploring_2020, krishna_hurdles_2021}. Furthermore, they fail to capture simple syntactic constructs and semantics properties \citep{lakretz_emergence_2019, lakretz_can_2021, baroni_linguistic_2020, lake_word_2021}.

%
% Transition
% What key differences remain between these two systems?
% What explain the different cognitive abilities of these two systems?

Here, we propose that these shortcomings are partly caused by an inherently short-sighted learning rule. Specifically, while these deep language algorithms are typically trained to predict words from closely surrounding contexts (e.g. predicting the very next word), we hypothesize that the human brain is tuned to forecast multiple levels of representations far-off in the future (Figure \ref{fig:fig1}).

% While deep language models are short-sighted, as focused on the very next word, we hypothesize that the brain makes long-range and abstract predictions.

% We hypothesize that the brain does not solely focus on predicting the next word but makes longer-term and more abstract predictions.

% Representation of what's expected to occur
% Forecast == estimate of future events -> forecast representation

% prediction / forecast / expectation (representation)

% \jr{
% % Question 
% Here, we argue that DLM's learning rule is fundamentally short-sighted. It only predict the following word, while the brain makes longer-term and more abstract predictions.
% While humans constantly anticipate high-level language representations, these algorithms are trained to predict words, although their individual occurrence rapidly becomes non-deterministic in the future. 
% }

% \charlotte{
% Here, we investigate one major difference: while DLMs are trained to predict one word given its context, we hypothesize that the brain makes longer-term and more abstract predictions. Specifically, we hypothesize that there exist anticipation representations in the brain when processing the words $w_1, \dots w_n$, which are absent from DLMs' activations when processing the same words. 
% }

% Methods
To test this hypothesis, we analyse the brain signals of 304 subjects listening to short stories, while their brain activity was being recorded with fMRI \cite{nastase_narratives_2020}. After confirming that deep language models linearly map onto these brain signals \cite{schrimpf_artificial_2020, caucheteux_disentangling_2021,toneva_interpreting_2019}, we show that adding forecast representations to the models improves the brain-mapping. 
%We systematically vary the distance of future words, and the nature of the representation. 
% We show that adding forecast representations significantly improves the mapping with the brain, up to eight words in the future ($\approx 4$s).
%
This improvement (i) varies across regions, (ii) is maximal in associative cortices and (iii) depends on deep semantic forecasting. 

%This result confirms that, unlike modern deep algorithms, the human brain makes long-range and more abstract predictions. 
%Overall, this study provides empirical evidence of long-range predictive coding, and thus call for long-sighted learning rules in deep learning. 

% These results suggest that current DLMs lack the anticipation power of the brain, and could benefit from non-auto-regressive learning objectives. While they are good next-word predictors, they would also be myopic and fail to predict the more distant future like the brain does.


% OLD 

% % Recent progress in SSL 
% \dropcap{I}n less than three years, Deep Language Algorithms have made considerable progress in text generation, translation and completion \cite{vaswani_attention_2017,radford_language_nodate, brown_language_2020}, thanks to a simple learning rule: predicting words from their context. 
% %
% % Predict brain activity 
% Moreover, the activations of these algorithms linearly map onto brain responses to spoken and written language (fMRI \cite{toneva_interpreting_2019, schrimpf_artificial_2020}, MEG \cite{toneva_interpreting_2019, caucheteux_language_2020} and ECoG \cite{goldstein_thinking_2021}). 

% % Limitations
% Still, the gap between machines and humans remains wide open: current language models fail to compete with humans on tasks such as story generation, summarization, dialogue and long-form question answering \cite{holtzman_curious_2020, wiseman_challenges_2017, thakur_beir_2021, raffel_exploring_2020, krishna_hurdles_2021}. 
% %
% % Transition
% What key differences remain between these two systems?

% While deep language models are short-sighted, as focused on the very next word, we hypothesize that the brain makes long-range and abstract predictions.

% % Methods
% To test this hypothesis, we analyse the brain signals of subjects (n=304) listening to stories, while their brain activity is recorded using fMRI \cite{nastase_narratives_2020}. We first replicate previous studies and quantify the extent to which the activations of an auto-regressive model, GPT-2, map onto brain activity \cite{schrimpf_artificial_2020, caucheteux_disentangling_2021}. Then, we test whether adding representations of future words improves the mapping. We systematically vary the distance of future words, and the nature of the representation. 

% We show that adding forecast representations significantly improves the mapping with the brain, up to eight words in the future ($\approx 4$s). This improvement is maximal (i) in associative cortices (superior temporal, inferior frontal, and parietal areas), and (ii) when adding the deep semantic representations from GPT-2. This result confirms that, unlike modern deep algorithms, the human brain makes long-range and more abstract predictions. Overall, this study provides empirical evidence of long-range predictive coding, and thus call for long-sighted learning rules in deep learning. 

% These results suggest that current DLMs lack the anticipation power of the brain, and could benefit from non-auto-regressive learning objectives. While they are good next-word predictors, they would also be myopic and fail to predict the more distant future like the brain does.


==> 41_discussion_old.tex <==
\section*{Discussion}

In this study, we track forecast representations in the brain of 304 subjects listening to short stories while recorded using fMRI. We show that, contrary to modern deep language models, the brain makes long-range ($d>5$) and abstract predictions. Critically, our results reveal a hierarchy of forecasts representations: from shallow and short-range forecasts in low-level regions to deep and long-range predictions in associative cortices. 

Our study contributes to a large body of work investigating the learning rule inherent to language processing. This question is ubiquitous in both Neuroscience and Machine Learning.

%Complements previous work in predictive coding in the brain % Ubiquitous
%The question of the learning rule performed by the brain
%This question is ubiquitous Neuroscience. 
In Neuroscience, the brain is known to spontaneously predict the very next word in response to both written and spoken sentences (fMRI \cite{willems_prediction_2016, lopopolo_using_2017, okada_neural_2018, shain_fmri_2019}, EEG \cite{heilbron_tracking_2019}), MEG \cite{mousavi_brain_2020} and  ECoG \cite{forseth_language_2020, goldstein_thinking_2021}).  However, these studies focused on (i) the short-range predictions of the very next word (although see \cite{wang_dynamic_nodate}) and (ii) the prediction's error (one scalar) as opposed to the forecast representations themselves (although see \cite{goldstein_thinking_2021}). Thus, our study complement previous work by analysing the\textit{ long-range }forecast \textit{representations} in brain responses to \textit{language}. 
% TODO: add comparison with the localized effects: IFG, 
Other studies have addressed the question of \textit{long-range} prediction during movie visioning \cite{lee_anticipation_2021} (fMRI), decision making (XXX) and multi-step planning (XXX) using highly controlled stimuli.

% Non-auto-regressive learning rules in Natural Language Processing
In Natural Language Processing, a growing body of work investigate long-range \cite{yang_xlnet_2020} and high-level learning rules \citep{clark_electra_2020}. 

[...]

% Building new architectures, analyse the causal relationship between long-range prediction and performance at language tasks is an important direction for future work. 


% Format of representation
Here, we not only highlight the brain's spontaneous predictions, but provide empirical evidence for the possible \textit{format} and \textit{nature} of these forecast representations. 

[...]

Overall, this study provides empirical evidence of long-range predictive coding in the human brain and calls for (1) non-auto-regressive, (2) long-range and (3) hierarchical learning rules in Machine Learning. 


% While we do not directly investigate the feedback \textit{errors}, but the forecast \textit{representations}, our study provides empirical evidence of hierarchical predictive coding in the brain, and complement previous work 



% Non-trivial dissociation between (i) the mapping between gpt2 and the brain (2) the regions where the forecast score 
% Provide evidence that GPT-2 lack the forecast representations of the brain. Pas les regions les mieux predites qui n'ont pas la signature de forecast la plus importante. Pre-frontal anticipte + loin et plus abstraite. 



%In line with previous studies, our work provides empirical evidence for predictive coding in the brain. When processing sentences, the brain is known to spontaneously predicts the very next word. fMRI \cite{willems_prediction_2016, lopopolo_using_2017, okada_neural_2018, shain_fmri_2019}, EEG \cite{heilbron_tracking_2019}), MEG \cite{mousavi_brain_2020} and  ECoG \cite{forseth_language_2020, goldstein_thinking_2021} analyses have shown that next-word surprisal predicts brain activity during language processing. Yet, these studies focused on the next-word prediction's \textit{error} (one scalar), as opposed to the \textit{anticipatory representations} themselves. While one study \cite{goldstein_thinking_2021} has directly tracked the representation of the incoming word in ECoG recordings using deep language models' activations, they did \textit{not} explore the differences between DLMs and the brain in encoding \textit{long-range} anticipatory representations. While the latter work emphasizes the \textit{similarities} between DLMs and the brain in \textit{next-word} prediction, we complement and qualify these findings by highlighting the \textit{differences} between the two systems in \textit{long-range} anticipation. 
% Two papers have addressed the question of \textit{long-range} anticipation during language comprehension \cite{wang_dynamic_nodate} (fMRI, MEG and EEG) and movie visioning \cite{lee_anticipation_2021} (fMRI) using highly controlled stimuli. Yet, the aim was not to compare brain activity with deep neural networks. Thus, our work  

%Echoes various attempts to  include non auto-regressive learning rule 
% In language Fan et al. XLNet, 
% In Vision ICCV paper with Lecun 
% Wav2Vec, first attempt 

% Sugggere different niveau d'abstraction dans la prediction. 

% Confirme les idees de predictive coding, mais premier resultat empire qui montre que les representations de predictions sont dans le meme format 
% Difference entre representation et information
% Format de Representation


%% Limitations
% Specific aspect of predictive coding: forecast \textit{representations} (as opposed to feedback errors)
% Low scores
% Ideal future vs. true future
% Do not directly investigate deep neural networks. Future work: building new architectures, analyse the causal relationship between long-range prediction and performance at language tasks. 

\subsection{Other possible organisation for the discussion}


Our study provides three main contributions. 

First, results show that the brain makes \textit{long-range} predictions. The brain is known to spontaneously predict the very next word [...]. Yet, long-range forecasts have been sparsely explored in the neuroscience of language. 

Second, the present study investigates the \textit{nature} of the forecast representation. [...] We show that future GPT-2 activations accurately account for forecasting in the brain. First study, to our knowledge, to highlight the possible format of the forecast representations. 

Third, the present study reveals a \textit{hierarchy} of predictions in the brain. [...] Not only do we highlight long range and abstract predictions, but investigate the interaction between both, and their spatial organisation in the brain. 

Our study contributes to a large body of work investigating the learning rule, and strengthens predictive coding theories. 

Predictive coding [...] 

In Neuroscience, evidence of prediction, feedback, (language, in vision, speech). [...]

In ML, recent work have explored new architectures and non-autoregressive learning rules [...]. Exploring new architectures and learning rule in an exciting future direction. 

Overall, 





==> notes.tex <==
% Then, we show that adding XXXXX representations from the n=XXX future words %improves this mapping.
% best account for brain responses.
%We quantify to what extent the brain encodes future events.

% If so, it would demonstrate that 
% Then, we concatenate ``anticipatory” representations to the latter GPT-2 activations, i.e. representations containing information about words that have not been pronounced yet (e.g. words $w_{n+1}, \dots w_{n+d}$).
% We systematically vary the anticipation distance $d$, the nature of the representation, and quantify the increase in our ability to predict brain activity. 

%Results
% We find that adding long-range  ($d>\,5$) anticipatory representations to those of GPT-2's largely improves the modeling of brain activity. 
% This improvement is (i) maximal in associative cortices (superior temporal, inferior frontal, and parietal areas), and (ii) when adding the deep semantic representations from GPT-2. 

% This result confirms that unlike modern DLMs the human brain makes long-range and more abstract predictions.

% This result highlight that modern DLMs fail to generate brain-like representations of the long-range and abstract future.

% This improvement highlights that (1) there exists anticipatory representations, present in the brain responses to word $w_1, \dots w_n$, but absent from DLMs activations of the same words and (2) that these missing representations can be partly accounted for by a high-level representation of future words. % This (2) point should be rephrased.

% \jr{
% % Conclusion / Ouverture
% Together, these results confirm that current DLMs lack the long-range anticipation power of the human brain.
% Finally, we formalize a brain-inspired framework to improve the fundamental myopia of current self-supervised AI algorithms.
% }

% \charlotte{
% Together, these results suggest that current DLMs lack the anticipation power of the brain, and could benefit from non-auto-regressive learning objectives. While they are good next-word predictors, they would also be myopic and fail to predict the more distant future like the brain does.
% }
% % Limitations relative to the question:



\paragraph{Limitations}\\
\textbf{We do:}
\begin{itemize}
\item show that there exists information encoded in GPT-2($w_1\dots w_{n+d}$)$[n+d] $that is present in the brain response to word $w_1\dots w_n$, but absent from GPT-2($w_1\dots w_n$)$[n]$. 
\end{itemize}
\textbf{We do NOT:}
\begin{itemize}
\item Quantify the degree of anticipation in deep networks (only the degree of ``brain-like'' anticipation).
\item Investigate the correlational/causal relationship between downstream tasks’ performance and anticipation power in deep networks (nor in humans)
\item Introduce a novel NLP architecture including long-range / abstract anticipation that improves downstream tasks. 
\item We only focus on shared/unshared anticipatory \textit{representations}, not on the \textit{feedback signal} relative to the prediction. 
\item We only focus on shared/unshared anticipatory \textit{representations} between the brain and DLMs, not their \textit{behavioral} differences. 
\item We do not explicitly orthogonalize GPT-2$[n+d] $) $\subset$ $\tilde{X}^{(d)}$ and GPT-2$[n] = X$. I.e. we say that $\tilde{X}^{(d)}$ are ``anticipatory'' representations, but they actually encode information about the past (because GPT-2 is fed with all the previous words). So the underlying hypothesis is that $\mathcal{R}(X)$ already account for all explained variance in the brain relative to the past and present representations. Thus, when calculating the anticipation score $\mathcal{A}^{(d)} =\mathcal{R}(X \oplus \tilde{X}^{(d)}) - \mathcal{R}(X) $, we already remove all the past and present information by subtracting $\mathcal{R}(X)$, and the gain is hypothesised to be independent to the brain response specific to the past and present words. The random GPT2 generated words controls partially helps to palliate this issue. 
\item We do not have access to an ideal model of the most likely future. Thus, we use the \textit{true} future as a proxy for the \textit{most likely} future and make the hypothesis that the subjects' stories are unsurprising. We make this assumption because we study subjects listening to \textit{natural} stories, i.e. without control for the sentences' surprisal. Theoretically, we could estimate \textit{a posteriori} the predictability of the subject's sentences. But, to our knowledge, even the best language models fail to estimate the predictability of long and true sentences. Since they are trained to assign the maximum probability to real sentences (e.g. from Wikipedia), the degree of surprisal in a real text is too fine to be captured by these models. 
\end{itemize}

% Narrow down the question
% Specifically, we do not compare the two systems' behavior, but study the intermediate representations they build to process language. 
\paragraph{Related work}
Recent neuro-scientific studies have provided strong evidence that, when processing sentences, the brain spontaneously predicts the incoming word. fMRI \cite{willems_prediction_2016, lopopolo_using_2017, okada_neural_2018, shain_fmri_2019}, EEG \cite{heilbron_tracking_2019}, MEG \cite{mousavi_brain_2020} and  ECoG \cite{forseth_language_2020, goldstein_thinking_2021} analyses have shown that next-word surprisal predicts brain activity during language processing. Yet, these studies focused on the next-word prediction's \textit{error} (one scalar), as opposed to the \textit{anticipatory representations} themselves. While one study \cite{goldstein_thinking_2021} has directly tracked the representation of the incoming word in ECoG recordings using deep language models' activations, they did \textit{not} explore the differences between DLMs and the brain in encoding \textit{long-range} anticipatory representations. \textbf{While the latter work emphasizes the \textit{similarities} between DLMs and the brain in \textit{next-word} prediction, we complement and qualify these findings by highlighting the \textit{differences} between the two systems in \textit{long-range} anticipation.}
Two papers have addressed the question of \textit{long-range} anticipation during language comprehension \cite{wang_dynamic_nodate} (fMRI, MEG and EEG) and movie visioning \cite{lee_anticipation_2021} (fMRI) using highly controlled stimuli. Yet, the aim was not to compare brain activity with deep neural networks. 

% \paragraph{Related work in NLP}
% Several studies have indirectly called for longer-term and abstract objective functions. Fan et al. \cite{fan_hierarchical_2018} have shown that predicting the text's \textit{structure} before its literal words improves the ability to generate stories. Non-auto-regressive objectives have been studied in the context of language modeling (XLNet + other papers), text tranlation (a lot of papers). 

\acknow{We thank Sam Nastase and collaborators for releasing the Narratives dataset, and for providing additional information on the fMRI data and comprehension questionnaires submitted to the subjects.}
\showacknow{}










% Motivation: 
% - major NLP progress
% - mapping w/ brain

% \paragraph{Extended abstract (Charlotte version)} \
% % Recent progress in SSL 
% \dropcap{I}n less than three years, Deep Language Models (DLMs) have made remarkable progress in language tasks hitherto considered specific to humans. These algorithms are trained with a simple auto-regressive objective (predicting a word from its previous context) and are able to generalise to a large variety of downstream tasks such as text generation, translation, completion and classification \cite{vaswani_attention_2017,radford_language_nodate, brown_language_2020}. 
% %
% % Predict brain activity 
% Critically, recent works have highlighted the unprecedented ability of DLMs to predict brain responses to spoken and written language recorded with various modalities (fMRI \cite{toneva_interpreting_2019, schrimpf_artificial_2020}, MEG \cite{toneva_interpreting_2019, caucheteux_language_2020} and ECoG \cite{goldstein_thinking_2021}), suggesting that the gap between language processing in brains and algorithms is narrowing. 

% % Limitations
% However, current DLMs still fail to compete with humans in certain complex tasks such as long story generation, text summarization, information retrieval and long-form question answering \cite{holtzman_curious_2020, wiseman_challenges_2017, thakur_beir_2021, raffel_exploring_2020, krishna_hurdles_2021}. 
% %
% % Transition
% This leads us to question the differences that remain between the two systems. 

% % Question 
% Here, we investigate one major difference: while DLMs are trained to predict one word given its context, we hypothesize that the brain makes longer-term and more abstract predictions. Specifically, we hypothesize that there exist anticipation representations in the brain when processing the words $w_1, \dots w_n$, which are absent from DLMs' activations when processing the same words. 

% % Previous work in Neuroscience 
% % The brain predict the incoming word (Goldsetein), and future events ().  
% % NLP
% % Generating the prompt before the text can help long story generation. Suggesting 

% % Methods
% To answer this question, we analyse the brain signals of 304 subjects listening to narratives, while their brain activity is recorded using fMRI \cite{nastase_narratives_2020}. We first replicate previous studies and quantify the extent to which the activations of an auto-regressive model, GPT-2, in response to words $w_1, \dots w_n$, linearly predict brain activity in response to the same words $w_1, \dots w_n$ \cite{schrimpf_artificial_2020, caucheteux_disentangling_2021}. Then, we concatenate ``anticipation” representations to the latter GPT-2 activations, i.e. representations containing information about words that have not been pronounced yet (e.g. words $w_{n+1}, \dots w_{n+d}$). We systematically vary the anticipation distance $d$, the nature of the representation, and quantify the increase in our ability to predict brain activity. 

% %Results
% We find that adding long-range  ($d>\,5$) anticipatory representations significantly increases GPT-2’s ability to predict brain activity. This increase is maximal in associative brain regions (superior temporal, inferior frontal, and parietal areas), and when adding the semantic/abstract representations extracted from deep layers of DLMs. This prediction discrepancy highlights that there exists anticipation representations, present in the brain responses to word $w_1, \dots w_n$, but absent from DLMs activations of the same words. 
% % Interestingly, these representations are of the same nature as DLM’s past and present representations, suggesting that current DLMs' activations could encode those if we slightly modified the learning objective. 

% % Conclusion / Ouverture
% Together, these results suggest that current DLMs lack the anticipation power of the brain, and could benefit from non-auto-regressive learning objectives. While they are good next-word predictors, they would also be myopic and fail to predict the more distant future like the brain does. 


==> two_figures.tex <==
% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\linewidth]{figures/Figure-1-long.png}
% %\includegraphics[width=11.4]{figures/Figure-1-long.png}
% \caption{\textbf{Experiment.} \textbf{A. } 101 subjects listen to narratives (70 min of unique audio stimulus in total) while their brain signal is recorded using functional MRI. At the end of each story, a questionnaire is submitted to the subject to assess their understanding, and the answers are summarized into a \emp{comprehension score} specific to each (narrative, subject) pair (grey box). In parallel (blue box on the left), we measure the alignment between the subject's brain activations and the activations of GPT-2, a deep neural network trained to predict a word given its past context, both elicited by the same narrative. To this end, a linear spatio (f) - temporal (g) model is fitted to predict the brain activity of one voxel $Y$, given GPT-2 activations $X$ as input. The degree of alignment, called "brain alignment score", is defined for each voxel as the Pearson correlation between predicted and actual brain activity on held-out data (cf Methods). Finally, we test the correlation between the comprehension scores of the subjects and their corresponding brain alignment using Pearsonr correlation (red). A positive $R$ score means that the common representations, shared across the brain and GPT-2, are key for the subjects to understand a narrative. \textbf{B.} GPT-2 alignment scores, averaged across fMRI voxels, for different activation spaces, from the non-contextualized word embedding ("layer 0") to the activations of the last layer ("layer 12"). The error bars refer to the standard error of the mean across (subject, narrative) pairs. \textbf{C.} GPT-2 alignment scores between the subjects' fMRI recordings, and the activations of the ninth layer of GPT-2, when presented with the same narratives. Alignment scores are averaged across subjects, narratives, and voxels within brain regions (157 regions within each hemisphere). Non-significant brain scores are not displayed, as assessed with a two-sided Wilcoxon test across (subject, narrative) pairs, testing whether the brain score is significantly different from zero (threshold: .05). The brain regions are defined by a subdivision of Destrieux Atlas (cf Methods). \textbf{D.} Comprehension scores across the seven narratives. Among the 27 stories of the initial dataset, seven narratives were selected for the analyses: they were followed by a questionnaire, and had variability in the answers (more than ten different answers across subjects). The 101 subjects do not systematically listen to the same narratives. Comprehension scores are standardized between 0 and 1, and measure the ability of one subject to understand one narrative.}
% \label{fig:fig1}
% \end{figure*}

% %\begin{SCfigure*}[\sidecaptionrelwidth][ht]
% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\linewidth]{figures/Figure-2.png}
% %\includegraphics[width=11.4cm]{figures/Figure-2.png}
% \caption{\textbf{Results}. \textbf{A.} Relationship between the subjects' understanding of the narratives (x-axis) and the degree of alignment between their brain activity and (i) phonological features, (ii) the non-contextual word embedding layer of GPT-2 and (iii) the ninth compositional layer of GPT-2 (y-axis). One blue dot is the brain alignment score (cf Figure\ref{fig:fig1}) for one (subject, narrative) pair, averaged across voxels.
% %The degree of alignment is measured by fitting a spatio-temporal linear model that predict fMRI voxels $Y$ given an activation space $X$. The degree of alignment is the Pearson correlation on held out data between predicted and actual brain signals. 
% $R$ scores (red) are the Pearson correlation between the comprehension scores (x-axis) and degree of alignment (y-axis). The p-value in grey indicates the significance of the Pearson correlation provided by scipy \cite{2020SciPy-NMeth}. In red, the corresponding regression line and the 95\% confidence interval of the regression coefficient. \textbf{B.} $R$ scores between brain alignment and comprehension for phonological, word embedding and GPT-2 features. Brain alignment scores are first averaged across voxels within brain regions (157 in each hemisphere), then correlated to the subjects' comprehension scores using Pearsonr correlation. Only significant $R$ scores are displayed, as assessed with Pearson's p-value as provided by scipy (threshold: .05). In yellow, the regions were the representations shared across GPT-2 and the brain are critical to understand narrative.\textbf{ C.} $R$ Correlation scores between the subjects comprehension and marginal brain alignment (i) $\mathcal{A}(\mathrm{word \ embedding}) - \mathcal{A}(\mathrm{phonological \ features})$ (ii) $\mathcal{A}(\mathrm{GPT-2}) - \mathcal{A}(\mathrm{phonological \ features})$ and (iii) $\mathcal{A}(\mathrm{GPT-2}) - \mathcal{A}(\mathrm{word \ embeddings})$.}
% \label{fig:fig2}
% \end{figure*}
